Multivariate Time Series Clustering for Environmental State Characterization of Ground-Based Gravitational-Wave Detectors

Gravitational-wave observatories like LIGO are large-scale, terrestrial instruments housed in infrastructure that spans a multi-kilometer geographic area and which must be actively controlled to maintain operational stability for long observation periods. Despite exquisite seismic isolation, they remain susceptible to seismic noise and other terrestrial disturbances that can couple undesirable vibrations into the instrumental infrastructure, potentially leading to control instabilities or noise artifacts in the detector output. It is, therefore, critical to characterize the seismic state of these observatories to identify a set of temporal patterns that can inform the detector operators in day-to-day monitoring and diagnostics. On a day-to-day basis, the operators monitor several seismically relevant data streams to diagnose operational instabilities and sources of noise using some simple empirically-determined thresholds. It can be untenable for a human operator to monitor multiple data streams in this manual fashion and thus a distillation of these data-streams into a more human-friendly format is sought. In this paper, we present an end-to-end machine learning pipeline for features-based multivariate time series clustering to achieve this goal and to provide actionable insights to the detector operators by correlating found clusters with events of interest in the detector.

==> intro_old.tex <==
Multivariate timeseries (MVTS) data is ubiquitous in our current times of \red{insert some buzzwords here like IoT, health sensors, or something} and thus the multivariate timeseries classification (MTSC) problem is robustly studied in the timeseries analysis community \red{citations needed} with recent resurgence of interest in multivariate timeseries anomaly detection (MTAD) \red{citations needed}. To undertake research in building faster, more scalable \red{add more buzz words here} methods for the classification task, using both traditional as well as deep learning approaches, the community heavily relies on a set of diverse datasets that have been painstakingly put together in the UCR/UEA MTSC archive\cite{bagnall2018uea} while for the anomaly detection task, a variety of datasets have been described and released in recent publications \cite{tafazoli2023matrix}\cite{yeh2023sketching} and it is presumed that at some point in the future an archive similar to the UCR/UEA MTSC archive would be created for MTAD. Curating such high quality labelled multivariate datasets is a non-trivial undertaking and in \cite{bagnall2018uea}, the authors describe in detail how a certain dataset was created along with the class labels as an outcome of data collection done via active experimentation.

It is often the case that certain scientific domains, like particle physics and gravitational-wave astronomy, that employ large-scale infrastructure to do their science have a vast quantity of historical recordings of MVTS data that has been passively collected from a variety of sensors deployed across the infrastructure for monitoring and diagnostic purposes. In the present day, the domain experts are seeking to employ machine learning techniques to put this archived data to good use and gain actionable insights into potentially improving their experimental apparatus. This case is somewhat different from the active experimental setups which are used to create most of the datasets in the UCR/UEA MTSC archive where the class labels for each MVTS sample is assigned manually by construction of said sample. The domain experts who own such passively collected historical data stores typically do not provide a machine learning expert with the trifecta of - 1. a well-defined supervised machine learning task like classification or anomaly detection, 2. a task-specific dataset with ground-truth labels, and 3. downstream evaluation tests to validate the output of a machine learning pipeline (see section \ref{subsec:down_eval}). Therefore, to apply machine learning in such domains, a machine learning expert has to begin with unsupervised techniques like clustering. Moreover, the domain experts are not merely interested in a highly performant machine learning pipeline in terms of, say, classification accuracy or clustering quality or inference speed but an \textit{interpretable} one that can provide domain expert-friendly actionable insights.

In this paper, we present a case study of building an end-to-end multivariate timeseries analysis pipeline for seismic state characterization for ground-based gravitational wave observatories like the Laser Interferometer Gravitational wave Observatory (LIGO) - from formulating a machine learning task to defining domain-specific downstream validation tests to examine the output of such a tool to provide actionable insights to the detector operators. The task at hand, as described to the machine learning expert by a domain expert, is to \textit{identify known seismic phenomenon viz. earthquakes, microseisms, human activity in measurements made by the network of seismometers deployed at the detector site and assign an interpretable label to each point in time identifying combinations of phenomena and location where they are active}.

\textbf{Our main contribution are:}
\begin{itemize}
    \item \red{TBD}
    \item \red{TBD}
    \item \red{TBD}
\end{itemize}

The rest of this paper is organized as follows. In section \ref{background} we provide a brief background on gravitational wave astronomy and the state-of-the-art detectors that enable it, followed by a review of the existing work related to seismic state characterization. Section \ref{method} is a deep dive on the four modules of the proposed pipeline. We present results on a real LIGO dataset in section \ref{results} to demonstrate this pipeline in action. Finally, we conclude this paper in section \ref{conclusion}.
